Did the Model Understand the Question?

We analyze state-of-the-art deep learning models for three tasks: question answering on (1) images, (2) tables, and (3) passages of text. Using the notion of \emph{attribution} (word importance), we find that these deep networks often ignore important question terms. Leveraging such behavior, we perturb questions to craft a variety of adversarial examples. Our strongest attacks drop the accuracy of a visual question answering model from $61.1\%$ to $19\%$, and that of a tabular question answering model from $33.5\%$ to $3.3\%$. Additionally, we show how attributions can strengthen attacks proposed by Jia and Liang (2017) on paragraph comprehension models. Our results demonstrate that attributions can augment standard measures of accuracy and empower investigation of model performance. When a model is accurate but for the wrong reasons, attributions can surface erroneous logic in the model that indicates inadequacies in the test data.

==> attack.tex <==
\section{Crafting Adversarial Inputs}\label{sec:attacks}

We now describe three different attacks against NP that introduce semantically
irrelevant changes to the input, but cause NP to produce the wrong answer.
The attacks leverage weaknesses in 
NP's operator and column selection logic as surfaced by
the attributions.

\subsection{Fluff word deletion attacks}
On examining the attributions for operator and column selection
to question words (see Section~\ref{sec:understanding:observations}), we found
that sometimes an operator selection is based on fluff
words (also called \emph{stop words}) like: ``a'', ``at'', "the'', etc. For instance, 
in the question, ``what ethnicity is at the top?'', the operator
$\opnext$\footnote{The selection of the \opnext\ operator in answering
this question is surprising and non-robust in its own right; we
leverage this kind of non-robustness in our table row reordering attacks}
 is triggered on the word ``at''. Dropping the word ``at'' from
 the question changes the operator selection and causes NP to
 return the wrong answer. For more such examples, please refer to the
 attributions available on our
github page~\newcite{github-repo}.

Selecting operators based on fluff words is not robust.
In real search usage logs, users often phrase their questions concisely by dropping fluff words.
For instance, the user may simply say ``top ethnicity''.
To measure the extent of this non-robustness, we drop fluff words
from questions in the dev dataset that were originally 
answered correctly and test NP on them.
The fluff words to be dropped were manually selected and are
shown in the supplementary material~\ref{appendix:section:fluffwords}, Figure~\ref{fig:fluffwords}. 
By dropping
fluff words, the accuracy drops from $\devaccuracy$\% to $28.60$\%.
It may be possible to defend against such examples by generating synthetic training data, 
and re-training the network on it. 
                                
    
\subsection{Question concatenation attacks}
In these attacks, we either suffix or prefix a content-free phrase to the question. The phrase
is picked by using semantically irrelevant trigger words for operator selection. 
We manually ensure that the phrases are content-free. 

Table~\ref{tbl:prefixattacks} describes our results.
It shows $6$ phrases and the corresponding
drop in accuracy  on the dev dataset when the phrase is concatenated as a
prefix or a suffix to the question\footnote{When concatenating the phrase, a
 comma is inserted between the question and the phrase, and the punctuation at the end
 of the question is left intact}. 
%The
%drop is accuracy is on top of the original accuracy of $\devaccuracy\%$
%on the dev dataset.

We now explain how we constructed the phrases. We first aggregated the top 
attributed words for various operator selections across the dev dataset;
see Supplementary Material~\ref{appendix:section:optriggers}, Table~\ref{tbl:optriggers}
The first phrase uses the
word ``not'' which occurs as a trigger for the operator \opnext\ but
its usage in the attack phrase is semantically irrelevant. The next three phrases involve
the words ``chart'', ``listed'' and ``same'' respectively. While ``chart'' is a trigger
for the operator \opfirst\ while ``listed'' and ``same'' are trigger for \opnext.
Recall from Section~\ref{sec:understanding} that these are all superfluous triggers in the questions
they were used. The next two phrases phrases use the words ``above'',  and ``at'' respectively.
These are all triggers for the operator \opgeq. However the phrases do not include
a metric bound, and therefore the words are in fact invalid triggers for the operator in the
context of the phrase.

The union of the $6\times2=12$ attacks drop the accuracy on the dev dataset from 
$\devaccuracy\%$ to $5.01\%$. The attacks from the three phrases ``in this chart'', 
``among the rows listed'', and ``in not a lot of words'' alone drop the accuracy $7.42\%$.

We were surprised by the large drop in accuracy because all words in the original question 
remain intact. These attacks demonstrate a different kind of weakness compared to the one 
exploited by the fluff word attacks. 
%We note that the resulting questions from these attacks could occur in practice in a
%conversational assistant setting within a real product.
%It is plausible that these attacks could be mitigated by generating synthetic training data
%with negative examples, and re-training the network on it. In this sense, the attributions are
%useful in construction of such a training dataset.

\subsection{Row reordering attacks} 
We found that NP often got the question right by leveraging artifacts of the table.
For instance, the operators for the question
``which nation earned the most gold medals'' are \opresetselect, \opprev, \opfirst\ and \opprint. 
The \opprev\ operators essentially excludes the last row from the answer computation. 
It gets the answer right for two reasons: (1) the answer is not in the last row, and
(2) rows are sorted by the values in the column ``\ms{gold}''. 
%The presence of a ``\ms{total}'' row in the table can interfere with applying 
%operators such as \opmax\ and pre-applying \opprev\ to exclude the last row 
%(where ``\ms{total}'' rows are typically found) can be beneficial. 
%However, we found that NP excludes the last row even when there is 
%no ``\ms{total}'' row in the table and gets the right answer. 
%This works because, generally speaking, there is only a small chance of the answer being in the last row. 
Another example is questions like ``nick roach was signed the same day as what other player?"
that involve a ``same'' comparison. Such questions cannot be handled by NP's
operator language. Instead, NP uses the
program [\opwordmatch, \opnext, \opfirst, \opprint] to (non-robustly)
answer these questions, again relying on row ordering in the table.
%Our attributions
%confirm this by identifying ``same'' as a trigger for the operator \opnext.

In general, a question-answering system should not rely on row ordering as there are multiple
ways in which a table can be ordered. 
To quantify the extent of these kinds of biases, we carried out the following perturbations on tables:
(1) shuffled all rows excluding the last one, (2) Moved the correct answer to the first row,
%except when the table contains a \ms{total} row, 
(3) Moved the correct answer to the last row 
%, except when the table contains a \ms{total} row.
We do not apply these attacks when the question refers to the relative ordering of rows in the table. 
Specifically, we exclude questions which contain any of:  ``first'', ``last'', ``next'', ``previous'', ``before'',
``after'', ``above'', ``below''. Table~\ref{tbl:rowperturb} shows our results. We manually verified that none of the
perturbations affected the table semantics. We see that only 29.05\% of the questions pass all the three attacks. 

\begin{table}
    \centering \small 
    \begin{tabular}{@{}l@{}ll|ll@{}}
        \toprule
        \textbf{Attack Phrase} & \textbf{Prefix} & \textbf{Suffix} & \textbf{Attack} & \textbf{Acc.}\\
        \midrule
        ``in not a lot of words'' &  $-12.92\%$ & $-23.91\%$ & Original &  $\devaccuracy\%$ \\
        ``in this chart'' & $-2.89\%$ & $-4.23\%$  & Shuffle &  $31.47\%$ \\
        ``among these rows listed'' & $-3.42\%$ & $-7.31\%$ & Move last &  $30.29\%$ \\ 
        ``if its all the same'' & $-11.62\%$ & $-15.65\%$ &  Move first &  $32.56\%$  \\ 
        ``above all'' & $-7.17\%$ & $-14.02\%$ &  Union &  $29.05\%$ \\ 
        ``at the moment'' & $-2.47\%$ & $-7.62\%$ & & \\
        \bottomrule
    \end{tabular}
    \caption{\small Left: Drop in accuracy on dev dataset when various attack phrases are concatenated
    to the question as prefixes or suffixes. (Original accuracy: $\devaccuracy\%$). Right: Results of row reordering attacks}
\label{tbl:prefixattacks}
\label{tbl:rowperturb}
\vspace{-0.75cm}
\end{table}



%\begin{table}
%    \centering \small 
%    \begin{tabular}{ll}
%        \toprule
%        \textbf{Attack} & \textbf{Accuracy} \\
%        \midrule
%        Original &  $\devaccuracy\%$ \\
%        Shuffle &  $31.47\%$ \\
%        Move last &  $30.29\%$ \\
%        Move first &  $32.56\%$ \\
%        Union &  $29.05\%$ \\
%        \bottomrule
%    \end{tabular}
%    \caption{Results of row reordering attacks.}
%\label{tbl:rowperturb}
%\vspace{-3mm}
%\end{table}


\begin{remark}
To eliminate this kind of weakness, there are two steps one could potentially
take during
training of the DNN: (1) including perturbed versions of the tables in the training set,
and (2) constraining the DNN with rules. One example of a
rule is, ``Use operators \opfirst\ and \oplast\ only when synonyms of those words
appear in the question''. Both approaches have the common purpose of forbidding
operators such as \opfirst\ from being used when the question asks for a \opmax.
%     Note that the \opfirst\ operator is column-independent, i.e., it does not depend on the specific column it is paired with. When the model is disallowed from using such column-independent operators, the task becomes significantly more difficult, as, to get the correct answer, it should get both the operator and column right. 

\begin{remark}
    We tested our attacks on the state-of-the-art model [Krishnamurthy et al., EMNLP-2017] and found it to significantly drop accuracy. For instance, the “table perturbation”, "fluff word", and "question concatenation" attacks drop its dev accuracy by 5.2\%, 5.7\% and 24.5\% respectively. 
\end{remark}

\end{remark}


%\begin{itemize}
%\item Attributions => Attacks: methodology (fluff words, non-synonyms,
%  paraphrasing) and results
%\item Point out that these attacks hit on ``conceptual'' flaws in NP.
%  Contrast with the adversarial perturbation attacks on image models.
%\item Comment black box vs white box methods. Why attributions help?
%\item We tend to see ill-formed english in product logs..
%\item attack is not necessarily on the technology; it is possibly on
%  the training data
%\end{itemize}


==> related.tex <==
\section{Related Work}\label{sec:related}
\label{sec:related_work}
\subsection{Program analysis}\label{sec:relatedpl}
Our analysis method has two different connections with classic
program analysis. The first is a direct connection with
\emph{program slicing} which amounts to finding all statements in a program that
directly or indirectly affect a certain target variable (also
called \emph{slicing criterion})~\newcite{W81, AM90}. We effectively use slicing
to determine which inputs affect various output variables in NP; this is discussed in Section~\ref{sec:prelim}.
For instance, through slicing, we discover that only matches between the table 
and the question (and not the raw table contents) affect the operator and column
selection.
%Slices are 
%commonly examined while debugging programs to isolate cause
%of errors~\newcite{weiser-debugging}. 
%The first is a direct application of slicing in order to determine which inputs affect a 
%certain output variable in a DNN; this is discussed in Section~\ref{sec:prelim}.
%For instance, through slicing we discover that only matches between the table 
%and the question (and not the raw table contents) affect
%the operator and column selection.
%Such an application of slicing is relevant to other DNNs as well especially
%when understanding intermediate outputs. For instance, in convolutional
%networks, slicing can help determine which input pixels affect a certain
%intermediate convolution node.

The second is a somewhat subtle connection with \emph{path-sensitive} analysis of
programs. Different control-flow paths in a program, presumably, carry different semantic
influences on a target variable. Path-sensitive methods~\newcite{BA98} examine data dependencies
separately along individual control-flow paths. Unlike programs, DNNs typically do not contain 
explicit control-flow. 
However, if we think of a DNN as a continuous relaxation of an underlying
(but unknown) discrete program then the control-flow logic may still be present \emph{softly}
in the dataflow paths. To illustrate this point, consider discrete control-flow of the form 
$\mbox{\tt if}~P(x)~\mbox{\tt then}~F(x)~\mbox{\tt else}~G(x)$. This may be relaxed
as $(1 - P^{c}(x)).F^{c}(x) + P^{c}(x).G(x)$, where $P^{c}$, $F^{c}$ and $G^{c}$ are themselves
continuous relaxations of the functions $P$, $F$, and $G$.  The {\tt if} branch now corresponds to the 
dataflow paths for the expression $(1 - P^{c}(x)).F^{c}(x)$. 

Following this
intuition, in Section~\ref{sec:rules}, we posit that different groups of dataflow paths
in the network may capture different semantic influences. Analogous to path-sensitive analysis,
we extended the Integrated Gradients method to compute attribution along separate
dataflow paths. In general, it is not a priori clear how to group the
  paths, especially since the underlying discrete program is unknown. In our case, we manually
  abstracted NP (Listing~\ref{lst:np-abstraction}) based on our understanding of its
  architecture, and speculated that a certain dataflow path may carry synonym influence.

\subsection{Analysis techniques for DNNs}
Similar to Integrated Gradients, there are many other methods that could be used
to attribute a DNN's prediction to its input features~\newcite{BSHKHM10,SVZ13,SGSK16,BMBMS16,SDBR14}. 
We chose Integrated
Gradients due to its ease of implementation and its axiomatic justification; 
we refer to the original Integrated Gradients paper~\newcite{STY17} for a detailed comparison with other attribution methods.
A novel contribution of this paper is the extension of the Integrated Gradients method
to specifically attribute through certain dataflow paths in the network.

There has been work around verification of properties of DNNs, for instance~\newcite{KBDJK17}.
%In contrast to our work, the DNN they analyze has a simpler topology, and the task that they
%analyze has simpler semantics that can be formulated as a safety property. 
In contrast to our work, the DNNs they analyze have a simpler topology, and the properties being verified
are well-formulated safety properties. Consequently, their guarantees are cleaner. 
The complexity of
our analysis stems from the hardness of stating analogous properties for our network and task.
It is possible that our path-sensitive dataflow analysis can be combined with their method.

\subsection{Papers from PLDI reviews}

\newcite{ribeiro2016should} proposes a method called LIME which approximates black-box models locally with sparse linear models. "Locality" is determined by perturbing a given input in $\Re{R}^n$ via zeroing out few of the coordinates.
 For text classification, this means dropping out some of words as perturbations. 
Input here is bag-of-words. They show that few of the classes are being triggered by fluff words such as "by". 
For images, it means graying out patches or "super-pixels" of the image
Evaluation of their method is done by interpreting already interpretable models such as logistic regression and comparing the extracted set of most important features
They compare their method to Parzen, another interpretability method based on computing gradients
Discussion on "do explanations lead to insights?"

\newcite{yaghmazadeh2017sqlizer} Paper summary
- Task: translate natural language question into SQL query
- Use semantic parsing to first synthesize likely program sketches, which may have English hints in place of column names.
- Use word2vec to identify relevant column names, primary keys, etc corresponding to the English hints
- If program fails, perform repair by splitting string arguments in clauses, etc. 
- In an Error Analysis section (Sec 9.2), they attribute failure of queries to bad similarity scores between potentially relevant words in word2vec. E.g. "star"--"rating". They suggest using embeddings customized to domain. 



\newcite{lakkaraju2017interpretable} Paper summary
- Interpretation of a black box model in terms of a set of predicates such as "age >= 50"
- For classification tasks, class predictions by a blackbox model is interpreted by a given set of predicates 
- Compare this to LIME, where interpretations for each individual inputs are determined
- An optimization is crafted so as to minimize a few metrics such as number of predicates, ambiguity, etc.
- Experiments compare to LIME and Bayesian Decision Lists
- The blackbox model chosen for expts is one that takes as input heath records, demographic info and predicts whether an individual is "depressed" or "healthy"
- This method is only applicable to classification problems. In addition, their method assumes that a set of predicates is a priori provided. Their method has been evaluated on only one 5-layer feedforward network performing binary classification. While they do penalize number of predicates in the approximation, it is still unclear how their method performs when the input and output spaces are orders of magnitude larger as in text models.


\newcite{bastani2017interpretability} Paper summary:
- They build a decision tree which approximates a given model. 
- Technique is similar to standard method for building a Classification or Regression Tree
- Input space is modeled as mixture of Gaussians.
- Experiments are done on very simple models
- They build a greedy decision tree by assuming a Gaussian distribution of the input data. It is not directly applicable to question answering models such as Neural Programmer as the input data (text corpora) have Zipfian distributions. It is also unknown what kind of distributions inputs such as “table matches” follow, which hinders applicability

\subsection{Adversarial analysis}
Recently, there have been a number of techniques for crafting adversarial 
attacks against DNNs. Most of these techniques are targeted at image
networks, where, applying a tiny perturbation to the
image drastically changes its prediction. Here the image does not visually change. There is no analog of such attacks for text. In our attacks, the question does perceptibly change, but there is no change in the semantics.

Adversarial attacks on reading comprehension systems were recently
considered in~\newcite{JL17}. Here, the system answers questions about a paragraph of text.
These attacks involve extending a paragraph with
an irrelevant sentence which causes the system to change its answer. 
Our attacks are different from these in two ways. First, some of our attacks modify the question, whereas all their attacks modify the paragraph text (analogous to our tables). Second, their attacks are black box, while our attacks leverage the network's weaknesses (visible via the attributions) to handcraft an attack.
%They note that ``high-precision paraphrase generation is challenging, as most edits to a sentence do actually change its meaning''. We get around this by using our knowledge of the network's weaknesses (visible via the attributions) to handcraft an attack; this is the second difference--their attacks are black box.

\subsection{Rule extraction}
The idea of extracting symbolic rules from neural networks is not
new~\newcite{craven1993learning,thrun1994extracting}.
More recently,~\newcite{murdoch2017automatic} developed techniques to
extract rules from complex LSTM networks. Penkov et
al.~\newcite{penkov17explaining} induce LISP-like programs from the
observed state transitions of a Deep Q-network.
For a more thorough discussion, see the surveys
by Jacobsson~\newcite{jacobsson2005rule} and
Hailesilassie~\newcite{hailesilassie16rule}.


\subsection{Neural program synthesis}
Neural Programmer is part of a larger class of techniques that
use deep learning for program synthesis. The idea is to train
a DNN to predict a program from a given specification. The specification may be in
 natural language (as in NP), or input-output-examples.
Important networks in this area include RobustFill~\newcite{DUBSMK17},
Neuro-Symbolic Program Synthesis~\newcite{PMSLZK17}, DeepCoder~\newcite{BGBNT17},
and many others; see~\newcite{SK17} for a survey. Our analysis method applies to 
such program synthesis networks as well. For instance, we could use attributions
to understand what parts of the input specification triggers the selection of various
statements in the program. A related class of networks is those that perform
\emph{neural program induction}~\newcite{KAS16, JM15, GWD14}. Here, conditioned
on a specification, the network learns to predict the output for a given input; the program
logic stays implicit in the network. Similar to NP, these networks typically have ``controller''
RNN that (softly) applies an operation on the input at each step. Our analysis method
could help understand the decisions made by the controller by attributing them
to features of the input.

